ImageNet3D: Towards General-Purpose Object-Level 3D Understanding

A vision model with general-purpose object-level 3D understanding should be capable of inferring both 2D (e.g., class name and bounding box) and 3D information (e.g., 3D location and 3D viewpoint) for arbitrary rigid objects in natural images. This is a challenging task, as it involves inferring 3D information from 2D signals and most importantly, generalizing to rigid objects from unseen categories. However, existing datasets with object-level 3D annotations are often limited by the number of categories or the quality of annotations. Models developed on these datasets become specialists for certain categories or domains, and fail to generalize. In this work, we present ImageNet3D, a large dataset for general-purpose object-level 3D understanding. ImageNet3D augments 200 categories from the ImageNet dataset with 2D bounding box, 3D pose, 3D location annotations, and image captions interleaved with 3D information. With the new annotations available in ImageNet3D, we could (i) analyze the object-level 3D awareness of visual foundation models, and (ii) study and develop general-purpose models that infer both 2D and 3D information for arbitrary rigid objects in natural images, and (iii) integrate unified 3D models with large language models for 3D-related reasoning.. We consider two new tasks, probing of object-level 3D awareness and open vocabulary pose estimation, besides standard classification and pose estimation. Experimental results on ImageNet3D demonstrate the potential of our dataset in building vision models with stronger general-purpose object-level 3D understanding.

==> tables/exp_probe_full.tex <==
\begin{table}[t]
    \centering
    {\small
    \begin{tabular}{lccccc}
        \toprule
        Encoder Model & Architecture & Supervision & Dataset & Acc@$\pi/6$ & Acc@$\pi/18$ \\
        \midrule
        DeIT III & ViT-B/16 & Classification & ImageNet-21k \\
        DINO \cite{caron2021emerging} & ViT-B/16 & SSL & ImageNet-1k \\
        DINO v2 \cite{oquab2023dinov2} & ViT-B/14 & SSL & LVD-142M \\
        \bottomrule
    \end{tabular}}
    \vspace{.1in}
    \caption{Quantitative results on probing of object-level 3D awareness.}
    \label{tab:my_label}
\end{table}

